Solving Data-centric Tasks using Large Language Models

Large language models (LLMs) are rapidly replacing help forums like StackOverflow, and are especially helpful for non-professional programmers and end users. These users are often interested in data-centric tasks, such as spreadsheet manipulation and data wrangling, which are hard to solve if the intent is only communicated using a natural-language description, without including the data. But how do we decide how much data and which data to include in the prompt? This paper makes two contributions towards answering this question. First, we create a dataset of real-world NL-to-code tasks manipulating tabular data, mined from StackOverflow posts. Second, we introduce a cluster-then-select prompting technique, which adds the most representative rows from the input data to the LLM prompt. Our experiments show that LLM performance is indeed sensitive to the amount of data passed in the prompt, and that for tasks with a lot of syntactic variation in the input table, our cluster-then-select technique outperforms a random selection baseline.

==> improvements.tex <==
\section{Improvements, Experiments Plan}

\subsection{Results on large datasets from TabLLM}

Sample run on some large datasets from TabLLM, they have classification (yes/no) questions tasks but we can create like 10 example queries for data manipulation tasks adapted from theirs.

\subsection{Results on noisy versions of SOFSet}

\subsection{K-means/Affinity prop Clustering and Selection}
We need to evaluate against some other techniques to cluster + select tabular data and this could be a direction. Also check out PCA which is a dimensionality reduction.

\subsection{LLMs-based Summarization}
   guided summary - ask the LLM queries related to the data for \eg, what are the most relevant features given the query then compute meta data related to the selected features! \eg 20\% of rows have sales above 1000. Meta data computation - count of Unique Values, distribution information, trends and patterns, summary statistics

\subsection{Clearer Metrics for Compression}
We need better metrics for showing the prompt efficiency since that is a core of the paper for \eg size of the prompt and inference time efficiency.

\subsection{Error Analysis with examples}
